Learning Robust Variational Information Bottleneck with Reference

We propose a new approach to train a variational information bottleneck (VIB) that improves its robustness to adversarial perturbations. Unlike the traditional methods where the hard labels are usually used for the classification task, we refine the categorical class information in the training phase with soft labels which are obtained from a pre-trained reference neural network and can reflect the likelihood of the original class labels. We also relax the Gaussian posterior assumption in the VIB implementation by using the mutual information neural estimation. Extensive experiments have been performed with the MNIST and CIFAR-10 datasets, and the results show that our proposed approach significantly outperforms the benchmarked models.

==> backups/backup.tex <==
\section{Adaptation for Multi-Task Learning}
Different tasks are conditionally independent from each other. Let $I(Z;Y_k)$ denote the mutual information for the downstream task $Y_k$. In the same manner as the information bottleneck method, we can formulate MTL as the optimization problem as follows
\begin{align}
\label{Eq:MIB_1}
\text{max}  & ~ \sum_{k=1}^K I(Z;Y_k),   \\
\label{Eq:MIB_2}
\text{s.t.} & ~ I(Z;X) \leq I_C.
\end{align}

Similar to Eq.~(\ref{Eq:IB_Lag}), instead of solving the above constrained optimization problem directly, we deal with the following Lagrangian objective function
\begin{align}
\label{Eq:MTIB_Lag}
\mathscr{L}_{\text{MTIB}} = \sum_{k=1}^K I(Z;Y_k) - \beta I(Z;X).
\end{align}

Direct computing the mutual information $I(Z;Y_k)$ and $I(Z;X)$ in Eq.~(\ref{Eq:MTIB_Lag}) is a challenging task. Variational inference can be employed to approximate them. Firstly, with Assumption 1, we can derive a variational lower bound for $I(Z;X)$ as follow


\begin{align}
\label{Eq:Prob_Weighted}
\log \left\{ p(y, z)\right\}  & ~ = \sum_{k=1}^K \log \left\{ p(y_k,z;\sigma_k) \right\}  \nonumber  \\
& ~ = \sum_{k=1}^K \log \left\{ p(y_k|z;\sigma_k)p(z) \right\}, 
\end{align}
where $\sigma_k$ is a positive scalar used to explicitly indicate the homoscedastic uncertainty of downstream task $k$. 


Eq.~(\ref{Eq:MTIB_Lag}), the final loss function of the proposed MTVIB can be obtained
\begin{align}
\label{Eq:MTVIB_Loss_Final}
& \mathscr{L}_{\text{MTVIB}}  \nonumber \\
= & \frac{1}{N}\sum_{n=1}^{N}\mathop{{}\mathbb{E}_{\epsilon_z \sim p(\epsilon_z)}} \bigg [ \sum_{k=1}^{K} -\log \big\{ p_{\theta_k}\big(y_n|f_{\phi}(x_n,\epsilon_z)\big) \big\} \bigg]  
\nonumber \\  & \qquad  + \beta D_{\text{KL}}(p_{\phi}\big(z|x_n)||q(z)\big) \nonumber \\
= & \sum_{k=1}^{K} \Big[\frac{1}{\sigma^2_k} \mathscr{E}_{k} + \log \{ \sigma_k \} \Big] + \beta D_{\text{KL}}(p_{\phi}\big(z|x)||q(z)\big). 
\end{align}
where $N$ is the size of mini batch for Monte Carlo sampling. Similar to the VIB, in model testing, we sample the latent variable $z$ using encoder $p_{\phi}(z|x)$, then $z$ will be used as the input for decoders $p_{\theta_k}(y_k|z)$ whose outputs are our model's predictions.


\subsubsection{Results on MNIST}
\begin{table*}[ht!]
\caption{FGSM attack results on MNIST.}
\label{Tab:fgsm_mnist}
\centering
\begin{tabular}{|c|c|c|c|c|c|c|c|} \hline
 Method & Clean & $\epsilon=0.05$ & $\epsilon=0.1$ & $\epsilon=0.15$ & $\epsilon=0.2$ & $\epsilon=0.25$ & $\epsilon=0.3$ \\ \hline
 Baseline &\textbf{0.9933} &0.9339 &0.9088 &0.9024 &0.8917 &0.8767 &0.8637\\
 Distillation &0.9928 &0.9660 &0.9510 &0.9469 &0.9365 &0.9189 &0.8812 \\ 
 Adversarial &0.9922 &0.9856 &0.9799 &0.9735 &0.9651 &0.9531 &0.9441\\ 
 VIB-R &0.9918 &0.9721 & 0.9643 &0.9565 &0.9384 &0.9193 &0.8849 \\ 
 VIB-M &0.9922 &0.9699 &0.9627 &0.9556 &0.9406 &0.9141 &0.8948\\ 
 VIB-R(Ref) &0.9929 &0.9905 &0.9845 &0.9799 &0.9681 &0.9506 &0.9171 \\ 
 VIB-M(Ref) &0.9931 &0.9899 &0.9846 &0.9802 &0.9716 &0.9529 &0.9261 \\ 
 VIB-M(PGD) &0.9907 &0.9838 &0.9755 &0.9674 &0.9591 &0.9477 &0.9355\\ 
 %VIB-M(Ref+Adv) &0.9907 &0.9898 &\textbf{0.9877} &\textbf{0.9864} &\textbf{0.9841} &\textbf{0.9846} &\textbf{0.9798}  \\
 VIB-M(Ref+PGD) &0.9926 &0.9900 &0.9891 &0.9876 &0.9860 &0.9845 &0.9817  \\
 VIB-M(Ref+FGSM) &0.9928 &\textbf{0.9916} &\textbf{0.9893} &\textbf{0.9890} &\textbf{0.9868} &\textbf{0.9857} &\textbf{0.9851} \\   
 \hline
\end{tabular}
\end{table*}


The FGSM attack results on MNIST are exhibited in Table \ref{Tab:fgsm_mnist}. 

\begin{table*}[ht!]
\caption{PGD attack results on MNIST.}
\label{Tab:pgd_mnist}
\centering
\begin{tabular}{|c|c|c|c|c|c|c|c|} \hline
 Method & Clean &  $\epsilon=0.05$ & $\epsilon=0.1$ & $\epsilon=0.15$ & $\epsilon=0.2$ & $\epsilon=0.25$ & $\epsilon=0.3$ \\ \hline
 Baseline &\textbf{0.9933} &0.9267 &0.8813 &0.7288 &0.5138 &0.3666 &0.3546 \\ 
 Distillation &0.9928 &0.9374 &0.7944 &0.4080 &0.0991 &0.0289 &0.0226\\ 
 Adversarial &0.9922 &0.9851 &0.9753 &0.9641 &0.9477 &0.9298 &0.9225  \\ 
 VIB-R &0.9918 &0.9256 &0.4884 & 0.0634 &0.0081 &0.0033 &0.0035   \\ 
 VIB-M &0.9922 &0.9311 &0.6415 &0.1363 &0.0111 &0.0027 &0.0021  \\ 
 VIB-R(Ref) &0.9929 &0.9501 &0.8773 &0.6405 &0.3697 &0.2285 &0.2059 \\ 
 VIB-M(Ref) &0.9931 &0.9827 &0.9196 &0.6127 &0.3728 &0.3309 &0.3290  \\ 
 VIB-M(PGD) &0.9907 &0.9826 &0.9724 &0.9566 &0.9418 &0.9239 &0.9174 \\ 
 %VIB-M(Ref+Adv) &0.9907 &\textbf{0.9875} &\textbf{0.9836} &\textbf{0.9786} &\textbf{0.9749} &\textbf{0.9686}  &\textbf{0.9665} \\
 VIB-M(Ref+PGD) &0.9926 &\textbf{0.9895} &\textbf{0.9858} &\textbf{0.9793} &\textbf{0.9755} &\textbf{0.9697}  &\textbf{0.9675} \\
 VIB-M(Ref+FGSM) &0.9928 &0.9857 &0.9751 &0.9606 &0.9424 &0.9225 &0.9116 \\  
 \hline
\end{tabular}
\end{table*}


\begin{table*}[ht!]
\caption{PGD attack results on MNIST.}
\label{Tab:pgd_mnist}
\centering
\begin{tabular}{|c|c|c|c|c|c|c|c|} \hline
 Method & Clean &  $\epsilon=0.05$ & $\epsilon=0.1$ & $\epsilon=0.15$ & $\epsilon=0.2$ & $\epsilon=0.25$ & $\epsilon=0.3$ \\ \hline
 Baseline &\textbf{0.9933} &0.9264 &0.8707 &0.6437 &0.2541 &0.0530 &0.0174 \\ 
 Distillation &0.9928 &0.9376 &0.7679 &0.3021 &0.0177 &0.0004 &0.0001\\ 
 Adversarial &0.9922 &0.9839 &0.9742 &0.9627 &0.9448 &0.9152 &0.8913  \\ 
 VIB-R &0.9918 &0.9207 &0.4286 & 0.0241 &0.0004 &0.0000 &0.0000   \\ 
 VIB-M &0.9922 &0.9311 &0.6415 &0.1363 &0.0111 &0.0027 &0.0021  \\ 
 VIB-R(Ref) &0.9929 &0.9520 &0.8611 &0.5571 &0.1842 &0.0307 &0.0064 \\ 
 VIB-M(Ref) &0.9931 &0.9627 &0.7534 &0.3458 &0.1912 &0.1684 &0.1632 \\ 
 VIB-M(PGD) &0.9907 &0.9889 &0.9861 &0.9841 &0.9803 &0.9750 &0.9632 \\ 
 %VIB-M(Ref+Adv) &0.9907 &\textbf{0.9875} &\textbf{0.9836} &\textbf{0.9786} &\textbf{0.9749} &\textbf{0.9686}  &\textbf{0.9665} \\
 VIB-M(Ref+PGD) &0.9926 &0.9878 &0.9848 &0.9801 &0.9744 &0.9681 &0.9538 \\
 VIB-M(Ref+FGSM) &0.9928 &0.9857 &0.9740 &0.9549 &0.9313 &0.8915 &0.7926 \\  
 \hline
\end{tabular}
\end{table*}






\begin{table*}[ht!]
\caption{PGD attack results on MNIST.}
\label{Tab:pgd_mnist}
\centering
\begin{tabular}{|c|c|c|c|c|c|c|c|} \hline
 Method & Clean &  $\epsilon=0.05$ & $\epsilon=0.1$ & $\epsilon=0.15$ & $\epsilon=0.2$ & $\epsilon=0.25$ & $\epsilon=0.3$ \\ \hline
 Baseline &\textbf{0.9933} &0.9267 &0.8820 &0.7282 &0.4489 &0.1938 &0.0738 \\% 
 Distillation &0.9928 &0.9383 &0.7923 &0.4018 &0.0930 &0.0253 &0.0177\\ %
 Adversarial &0.9922 &0.9837 &0.9752 &0.9641 &0.9542 &0.9410 &0.9040  \\% 
 VIB-R &0.9918 &0.9251 &0.4942 &0.0616 &0.0038 &0.0001 &0.0001 \\% 
 VIB-M &0.9922 &0.9617 &0.7649 &0.3728 &0.2315 &0.1932 &0.1642  \\% 
 VIB-R(Ref) &0.9929 &0.9508 &0.8780 &0.6298 &0.3188 &0.1061 &0.0292 \\% 
 VIB-M(Ref) &0.9931 &0.9844 &0.9195 &0.6127 &0.3061 &0.2019 &0.1448  \\ %
 VIB-M(PGD) &0.9907 &0.9882 &\textbf{0.9875} &\textbf{0.9843} &\textbf{0.9818} &\textbf{0.9752} &\textbf{0.9499} \\ %
 VIB-M(Ref+PGD) &0.9926 &\textbf{0.9896} &0.9869 &0.9831 &0.9785 &0.9595 &0.9080 \\% all
 %VIB-M(Ref+PGD) &0.9893 &0.9865 &0.9844 &0.9795 &0.9771 &0.9636 &0.9286 \\% half
 VIB-M(Ref+FGSM) &0.9928 &0.9843 &0.9754 &0.9608 &0.9406 &0.9120 &0.8298 \\  
 \hline
\end{tabular}
\end{table*}


\iffalse
\begin{table}
\caption{Running time per epoch on CIFAR-10 (CPU: i7-9750H, GPU: RTX2060).}
\label{Tab:time_cifar10}
\centering
\begin{tabular}{|c|c|c|c|} \hline
 Method & Time per epoch & Total epoch & Total time\\ \hline
 Baseline &34.526s &200 &1.92h\\ 
 Distillation &66.351 &170 &5.05h \\ 
 Adversarial &502.349/273.049s &100 &9.77h \\ 
 Adv+Ref &349.456s & &h \\ 
 VIB-R &28.831 &250 &2.00h\\ 
 VIB-M & &\\ 
 VIB-R(Ref) &63.291 &300  \\ 
 VIB-M(Ref) &71.128 &200 \\ 
 VIB-M(PGD) &134.058 &300\\ 
 VIB-M(Ref+PGD) &376.235 &140\\ 
 VIB-M(Ref+FGSM) &143.916 &80 \\
 \hline
\end{tabular}
\end{table}
\fi




% \subsection{Ablation Study}

% \begin{table}[ht!]
% \small
% \caption{Performance improvements ($\%$).}
% \label{Tab:Ablation}
% \centering
% \begin{tabular}{ |c|c|c|c|} \hline
% Method & Using VIB & Using Adv & Using Reference\\ \hline
% MNIST (FGSM)   &1.46 &3.47 &1.53 \\ 
% MNIST (PGD)    &12.97 &131.22 &15.05\\ 
% CIFAR10 (FGSM) &-4.94 &-10.85 &4.92 \\ 
% CIFAR10 (PGD)  &20.41 &33.77  &22.36 \\ 
% \hline
% \end{tabular}
% \end{table}

\iffalse
\begin{table*}[ht!]
\small
\caption{Models' classification test accuracy results ($\%$) with the FGSM attack on the MNIST dataset.}
\label{Tab:fgsm_mnist}
\centering
\begin{tabular}{|l|c|c|c|c|c|c|c|} \hline
 Method & Clean & $\epsilon=0.05$ & $\epsilon=0.1$ & $\epsilon=0.15$ & $\epsilon=0.2$ & $\epsilon=0.25$ & $\epsilon=0.3$ \\ \hline
 
 Baseline &$99.20_{\pm0.05}$ &$93.64_{\pm0.18}$ &$91.03_{\pm0.28}$ &$89.76_{\pm0.22}$ &$88.73_{\pm0.22}$ &$87.94_{\pm0.11}$ &$86.57_{\pm0.18}$\\%
 
 Baseline(KD) &$99.28_{\pm0.04}$ &$96.61_{\pm0.06}$ &$95.17_{\pm0.09}$ &$94.33_{\pm0.19}$ &$93.39_{\pm0.31}$ &$91.20_{\pm0.21}$ &$88.35_{\pm0.22}$ \\% 
 
 Baseline(PGD) &$99.17_{\pm0.02}$ &\pmb{$98.54_{\pm0.03}$} &$97.92_{\pm0.08}$ &$97.18_{\pm0.06}$ &$96.40_{\pm0.09}$ &$95.40_{\pm0.12}$ &$94.36_{\pm0.06}$\\% 
 
 Baseline(REF) &\pmb{$99.35_{\pm0.02}$} &$97.00_{\pm0.07}$ &$96.10_{\pm0.21}$ &$95.56_{\pm0.07}$ &$94.88_{\pm0.20}$ &$93.47_{\pm0.23}$ &$91.27_{\pm0.24}$\\%
 
 Baseline(PGD+REF) &\pmb{$99.35_{\pm0.03}$} &$97.00_{\pm0.11}$ &$96.02_{\pm0.12}$ &$95.58_{\pm0.14}$ &$94.75_{\pm0.26}$ &$93.52_{\pm0.38}$ &$91.35_{\pm0.18}$\\%
 
 VIB-R &$99.10_{\pm0.05}$ &$97.24_{\pm0.05}$ &$96.52_{\pm0.20}$ &$95.52_{\pm0.20}$ &$94.20_{\pm0.12}$ &$91.44_{\pm0.26}$ &$88.44_{\pm0.34}$ \\% 
 
 VIB-M &$99.17_{\pm0.03}$ &$96.96_{\pm0.11}$ &$96.23_{\pm0.08}$ &$95.29_{\pm0.18}$ &$94.04_{\pm0.17}$ &$91.68_{\pm0.15}$ &$88.96_{\pm0.40}$\\% 
 
 VIB-R(REF) &$99.24_{\pm0.03}$ &$97.24_{\pm0.07}$ &$96.58_{\pm0.10}$ &$95.45_{\pm0.12}$ &$93.35_{\pm0.27}$ &$90.45_{\pm0.33}$ &$86.33_{\pm0.50}$\\% 
 
 VIB-M(REF) &$99.28_{\pm0.02}$ &$96.96_{\pm0.08}$ &$96.19_{\pm0.16}$ &$95.44_{\pm0.16}$ &$94.79_{\pm0.05}$ &$92.86_{\pm0.23}$ &$89.60_{\pm0.04}$\\ %
 
 VIB-M(PGD) &$99.04_{\pm0.05}$ &$98.37_{\pm0.04}$ &$97.61_{\pm0.08}$ &$96.79_{\pm0.08}$ &$95.86_{\pm0.13}$ &$94.73_{\pm0.06}$ &$93.41_{\pm0.10}$\\ %
 
 VIB-M(REF+FGSM) &$99.22_{\pm0.06}$ &$98.06_{\pm0.06}$ &$97.64_{\pm0.12}$ &$97.35_{\pm0.08}$ &$97.12_{\pm0.13}$ &$96.89_{\pm0.09}$ &$96.53_{\pm0.11}$\\   
 
 VIB-M(REF+PGD) &$99.13_{\pm0.04}$ &$98.48_{\pm0.08}$ &\pmb{$98.03_{\pm0.04}$} &\pmb{$97.79_{\pm0.07}$} &\pmb{$97.59_{\pm0.08}$} &\pmb{$97.35_{\pm0.05}$} &\pmb{$97.12_{\pm0.12}$} \\% all
 
 \hline
\end{tabular}
\end{table*}


%The FGSM attack results on MNIST are exhibited in Table \ref{Tab:fgsm_mnist}. 

\begin{table*}[ht!]
\small
\caption{Models' classification test accuracy results ($\%$) with the PGD attack accuracy on the MNIST dataset.}
\label{Tab:pgd_mnist}
\centering
\begin{tabular}{|l|c|c|c|c|c|c|c|} \hline
 Method & Clean &  $\epsilon=0.05$ & $\epsilon=0.1$ & $\epsilon=0.15$ & $\epsilon=0.2$ & $\epsilon=0.25$ & $\epsilon=0.3$ \\ \hline
 
 Baseline &$99.20_{\pm0.05}$ &$92.60_{\pm0.06}$ &$87.36_{\pm0.23}$ &$64.54_{\pm0.39}$ &$22.88_{\pm0.14}$ &$3.09_{\pm0.13}$ &$0.36_{\pm0.05}$ \\%
 
 Baseline(KD) &$99.28_{\pm0.04}$ &$93.71_{\pm0.10}$ &$76.74_{\pm0.13}$ &$30.88_{\pm0.12}$ &$1.98_{\pm0.08}$ &$0.01_{\pm0.01}$ &$0.00_{\pm0.00}$ \\% 
 
 Baseline(PGD) &$99.17_{\pm0.02}$ &\pmb{$98.44_{\pm0.07}$} &$97.51_{\pm0.05}$ &$96.47_{\pm0.01}$ &$94.68_{\pm0.09}$ &$92.57_{\pm0.07}$ &$88.34_{\pm0.09}$  \\%
 
 Baseline(REF) &\pmb{$99.35_{\pm0.02}$} &$95.45_{\pm0.05}$ &$88.99_{\pm0.18}$ &$60.79_{\pm0.17}$ &$15.14_{\pm0.11}$ &$1.39_{\pm0.06}$ &$0.14_{\pm0.01}$\\%
 
 Baseline(PGD+REF) &\pmb{$99.35_{\pm0.03}$} &$95.39_{\pm0.17}$ &$89.98_{\pm0.13}$ &$66.31_{\pm0.24}$ &$22.75_{\pm0.21}$ &$2.58_{\pm0.14}$ &$0.36_{\pm0.04}$ \\%
 
 VIB-R &$99.10_{\pm0.05}$ &$92.06_{\pm0.19}$ &$43.28_{\pm0.24}$ &$2.55_{\pm0.08}$ &$0.03_{\pm0.02}$ &$0.00_{\pm0.00}$ &$0.00_{\pm0.00}$ \\ %
 
 VIB-M &$99.17_{\pm0.03}$ &$93.39_{\pm0.08}$ &$61.25_{\pm0.19}$ &$8.81_{\pm0.11}$ &$0.03_{\pm0.01}$ &$0.00_{\pm0.00}$ &$0.00_{\pm0.00}$ \\%
 
VIB-R(REF) &$99.24_{\pm0.03}$ &$95.19_{\pm0.07}$ &$86.33_{\pm0.24}$ &$55.69_{\pm0.50}$ &$17.51_{\pm0.23}$ &$2.15_{\pm0.10}$ &$0.27_{\pm0.03}$ \\ %
 
VIB-M(REF) &$99.28_{\pm0.02}$ &$95.17_{\pm0.06}$ &$86.28_{\pm0.23}$ &$53.82_{\pm0.32}$ &$13.53_{\pm0.05}$ &$1.64_{\pm0.09}$ &$0.19_{\pm0.02}$ \\%
 
VIB-M(PGD) &$99.04_{\pm0.05}$ &$98.26_{\pm0.02}$ &$97.19_{\pm0.06}$ &$95.84_{\pm0.06}$ &$94.03_{\pm0.13}$ &$90.86_{\pm0.14}$ &$85.51_{\pm0.18}$ \\ %
 
VIB-M(REF+FGSM) &$99.22_{\pm0.06}$ &$97.41_{\pm0.12}$ &$96.79_{\pm0.07}$ &$95.99_{\pm0.10}$ &$95.03_{\pm0.09}$ &$92.99_{\pm0.27}$ &$86.95_{\pm0.16}$ \\% 
  
VIB-M(REF+PGD) &$99.13_{\pm0.04}$ &$98.24_{\pm0.06}$ &\pmb{$97.70_{\pm0.08}$} &\pmb{$97.36_{\pm0.08}$} &\pmb{$96.87_{\pm0.09}$} &\pmb{$96.01_{\pm0.06}$} &\pmb{$93.64_{\pm0.30}$} \\% all
 
 \hline
\end{tabular}
\end{table*}

%The PGD attack results on MNIST are exhibited in Table \ref{Tab:pgd_mnist}. 


%\pagebreak

%\subsubsection{Results on CIFAR-10}
 

\begin{table*}[ht!]
\small
\caption{Models' classification test accuracy results ($\%$) with the FGSM attack accuracy on the CIFAR-10 dataset.}
\label{Tab:fgsm_cifar10}
\centering
\begin{tabular}{ |l|c|c|c|c|c|c|c|} \hline
 Method & Clean & $\epsilon=0.01$ & $\epsilon=0.02$ & $\epsilon=0.03$ & $\epsilon=0.04$ & $\epsilon=0.05$ & $\epsilon=0.07$ \\ \hline
 
 Baseline &$92.88_{\pm0.13}$ &$86.36_{\pm0.14}$ &$83.67_{\pm0.18}$ &$81.68_{\pm0.23}$ &$79.99_{\pm0.18}$ &$78.52_{\pm0.14}$ &$75.28_{\pm0.18}$ \\%
 
 Baseline(KD) &\pmb{$93.41_{\pm0.06}$} &$84.34_{\pm0.24}$ &$80.42_{\pm0.20}$ &$77.58_{\pm0.29}$ &$75.44_{\pm0.30}$ &$73.56_{\pm0.19}$ &$70.03_{\pm0.36}$ \\%
 
 Baseline(PGD) &$90.24_{\pm0.19}$ &$84.71_{\pm0.22}$ &$79.36_{\pm0.31}$ &$75.49_{\pm0.21}$ &$72.72_{\pm0.11}$ &$70.48_{\pm0.17}$ &$67.78_{\pm0.21}$ \\%
 
 Baseline(REF) &$90.51_{\pm0.22}$ &$84.71_{\pm0.34}$ &$81.81_{\pm0.21}$ &$79.52_{\pm0.17}$ &$77.31_{\pm0.26}$ &$75.15_{\pm0.29}$ &$71.96_{\pm0.16}$\\  %
 
 Baseline(PGD+REF) &$87.11_{\pm0.08}$ &$83.05_{\pm0.21}$ &$79.29_{\pm0.04}$ &$76.40_{\pm0.17}$ &$73.91_{\pm0.22}$ &$71.77_{\pm0.14}$ &$68.13_{\pm0.35}$ \\%
 
 VIB-R &$90.57_{\pm0.07}$ &$84.66_{\pm0.32}$ &$81.24_{\pm0.14}$ &$78.66_{\pm0.27}$ &$76.47_{\pm0.19}$ &$74.84_{\pm0.25}$ &$71.72_{\pm0.27}$ \\ %
 
 VIB-M &$91.47_{\pm0.14}$ &$84.79_{\pm0.24}$ &$81.94_{\pm0.15}$ &$79.98_{\pm0.22}$ &$78.16_{\pm0.13}$ &$76.52_{\pm0.11}$ &$73.87_{\pm0.26}$ \\%
 
 VIB-R(REF) &$90.98_{\pm0.07}$ &$86.82_{\pm0.16}$ &$84.80_{\pm0.23}$ &$83.09_{\pm0.19}$ &$81.62_{\pm0.20}$ &$80.37_{\pm0.20}$ &$77.97_{\pm0.25}$ \\ %
 
 VIB-M(REF) &$91.49_{\pm0.05}$ &\pmb{$87.42_{\pm0.17}$} &\pmb{$85.32_{\pm0.13}$} &\pmb{$84.01_{\pm0.32}$} &\pmb{$82.42_{\pm0.26}$} &\pmb{$80.97_{\pm0.24}$} &\pmb{$78.84_{\pm0.20}$} \\ %
 
 VIB-M(PGD) &$74.55_{\pm0.03}$ &$69.43_{\pm0.26}$ &$63.74_{\pm0.26}$ &$58.88_{\pm0.28}$ &$53.87_{\pm0.31}$ &$49.67_{\pm0.28}$ &$42.96_{\pm0.20}$ \\ %
  
 VIB-M(REF+FGSM) &$87.29_{\pm0.09}$ &$83.62_{\pm0.19}$ &$81.56_{\pm0.18}$ &$80.11_{\pm0.09}$ &$78.61_{\pm0.16}$ &$77.48_{\pm0.18}$ &$75.20_{\pm0.23}$ \\%
 
 %VIB-M(Ref+PGD) &$89.57_{\pm0.16}$ &$86.24_{\pm0.13}$ &$83.69_{\pm0.18}$ &$82.06_{\pm0.17}$ &$80.23_{\pm0.36}$ &$78.78_{\pm0.30}$ &$76.44_{\pm0.20}$ \\%

 VIB-M(REF+PGD) &$89.57_{\pm0.16}$ &$86.24_{\pm0.13}$ &$83.69_{\pm0.18}$ &$82.06_{\pm0.17}$ &$80.23_{\pm0.36}$ &$78.78_{\pm0.30}$ &$76.44_{\pm0.20}$ \\%
 
\hline
\end{tabular}
\end{table*}

%The FGSM attack results on CIFAR-10 are exhibited in Table \ref{Tab:fgsm_cifar10}. 

\begin{table*}[ht!]
\small
\caption{Models' classification test accuracy results ($\%$) with the PGD attack accuracy on the CIFAR-10 dataset.}
\label{Tab:pgd_cifar10}
\centering
\begin{tabular}{ |l|c|c|c|c|c|c|c|} \hline
 Method & Clean & $\epsilon=0.01$ & $\epsilon=0.02$ & $\epsilon=0.03$ & $\epsilon=0.04$ & $\epsilon=0.05$ & $\epsilon=0.07$ \\ \hline
 
 Baseline &$92.88_{\pm0.13}$ &$77.28_{\pm0.18}$ &$63.96_{\pm0.26}$ &$46.42_{\pm0.28}$ &$27.18_{\pm0.25}$ &$15.49_{\pm0.38}$ &$5.58_{\pm0.13}$ \\%
 
 Baseline(KD) &\pmb{$93.41_{\pm0.06}$} &$76.23_{\pm0.13}$ &$51.26_{\pm0.09}$ &$32.97_{\pm0.21}$ &$24.64_{\pm0.19}$ &$20.23_{\pm0.23}$ &$14.93_{\pm0.23}$ \\ %
 
 Baseline(PGD) &$90.24_{\pm0.19}$ &$84.00_{\pm0.11}$ &$76.02_{\pm0.23}$ &$67.08_{\pm0.15}$ &$58.13_{\pm0.22}$ &$50.37_{\pm0.23}$ &$41.04_{\pm0.16}$ \\%
 
 Baseline(REF) &$90.51_{\pm0.22}$ &$71.88_{\pm0.32}$ &$57.66_{\pm0.40}$ &$41.69_{\pm0.26}$ &$28.29_{\pm0.17}$ &$19.80_{\pm0.22}$&$11.74_{\pm0.14}$\\%
 
 Baseline(PGD+REF) &$87.11_{\pm0.08}$ &$82.56_{\pm0.11}$ &$77.21_{\pm0.16}$ &$71.65_{\pm0.21}$ &$65.17_{\pm0.36}$ &$58.65_{\pm0.24}$ &$46.25_{\pm0.18}$ \\%
 
 VIB-R &$90.57_{\pm0.07}$ &$79.06_{\pm0.34}$ &$63.62_{\pm0.25}$ &$48.99_{\pm0.33}$ &$36.59_{\pm0.13}$ &$26.93_{\pm0.21}$ &$14.39_{\pm0.25}$ \\ %
 
 VIB-M &$91.47_{\pm0.14}$ &$79.61_{\pm0.15}$ &$68.18_{\pm0.29}$ &$62.47_{\pm0.41}$ &$57.98_{\pm0.10}$ &$52.23_{\pm0.16}$ &$40.10_{\pm0.33}$\\ %
 
 VIB-R(REF) &$90.98_{\pm0.07}$ &$79.87_{\pm0.06}$ &$69.35_{\pm0.30}$ &$62.58_{\pm0.23}$ &$56.57_{\pm0.15}$ &$51.90_{\pm0.44}$ &$44.82_{\pm0.34}$\\%
 
 VIB-M(REF) &$91.49_{\pm0.05}$ &$80.55_{\pm0.19}$ &$70.52_{\pm0.18}$ &$60.05_{\pm0.24}$ &$50.94_{\pm0.20}$ &$44.01_{\pm0.09}$ &$35.02_{\pm0.18}$ \\% 
 
 VIB-M(PGD) &$74.55_{\pm0.03}$ &$68.74_{\pm0.12}$ &$62.92_{\pm0.27}$ &$56.32_{\pm0.37}$ &$50.29_{\pm0.19}$ &$44.46_{\pm0.32}$ &$33.91_{\pm0.22}$ \\%
  
 VIB-M(REF+FGSM) &$87.29_{\pm0.09}$ &$82.47_{\pm0.11}$ &$77.22_{\pm0.18}$ &$71.54_{\pm0.34}$ &$66.11_{\pm0.33}$ &$60.35_{\pm0.18}$ &$50.94_{\pm0.29}$ \\%
 
 VIB-M(REF+PGD) &$89.57_{\pm0.16}$ &\pmb{$85.65_{\pm0.08}$} &\pmb{$80.92_{\pm0.13}$} &\pmb{$75.78_{\pm0.20}$} &\pmb{$69.86_{\pm0.20}$} &\pmb{$63.89_{\pm0.20}$} &\pmb{$54.00_{\pm0.19}$} \\ %

 \hline
\end{tabular}
\end{table*}

\fi
